scTree: Discovering Cellular Hierarchies in the Presence of Batch Effects in scRNA-seq Data

We propose a novel method, scTree, for single-cell Tree Variational Autoencoders, extending a hierarchical clustering approach to single-cell RNA sequencing data. scTree corrects for batch effects while simultaneously learning a tree-structured data representation. This VAE-based method allows for a more in-depth understanding of complex cellular landscapes independently of the biasing effects of batches. We show empirically on seven datasets that scTree discovers the underlying clusters of the data and the hierarchical relations between them, as well as outperforms established baseline methods across these datasets. Additionally, we analyze the learned hierarchy to understand its biological relevance, thus underpinning the importance of integrating batch correction directly into the clustering procedure.

==> Sections/related_work.tex <==
\section{Related Work}



%Deep exponential families for single-cell data analysis

%Reconstructing unobserved cellular states from paired single-cell lineage tracing and transcriptomics data





Hierarchical clustering algorithms are a frequently used technique for unraveling the intricate hierarchical structures inherent in biological data. Agglomerative hierarchical clustering algorithms~\citep{sneath1957application, Ward1963HierarchicalGT,murtagh2012algorithms} treat each data point as a separate cluster and progressively merge these clusters based on their proximity, as defined by a specific distance metric. Diverging from traditional agglomerative techniques, Bayesian Hierarchical Clustering~\citep{heller2005bayesian} introduces a probabilistic framework that utilizes hypothesis testing for cluster merging decisions. Divisive hierarchical clustering algorithms~\citep{kaufman2009finding}, the category which TreeVAE falls into, offer an alternative strategy, starting with a single cluster that encompasses all data points and iteratively dividing it into smaller clusters. The Bisecting-K-means algorithm~\citep{Steinbach2000ACO, Nistr2006ScalableRW} repeatedly applies k-means clustering to divide data into two parts. Relatedly, \citet{williams1999mcmc} learn a hierarchical probabilistic Gaussian mixture model. Further hierarchical probabilistic clustering methods include VAE-nCRP \citep{Goyal2017NonparametricVA, Shin2019HierarchicallyCR} and the TMC-VAE \citep{Vikram2018TheLP}. that use Bayesian nonparametric hierarchical clustering based on the nested Chinese restaurant process (nCRP) prior \citep{hierarchicalpriorBlei} or the time-marginalized coalescent (TMC). 

Various hierarchical clustering algorithms have emerged to address the unique challenges encountered in single-cell RNA sequencing (scRNA-seq) data analysis. \cite{lin2017cidr} proposed Clustering through Imputation and Dimensionality Reduction (CIDR), leveraging imputation techniques within a hierarchical framework to mitigate the impact of dropouts inherent in scRNA-seq data. \cite{morelli2021nested} presented Nested Stochastic Block Models (NSBM) and \cite{zou2021hgc} proposed Hierarchical Graph-based clustering (HGC), both offering methods for hierarchical clustering directly on the k-nearest neighbor graph of cells, bypassing the count matrix. Additionally, scDEF, a method introduced by \cite{Ferreira2022.10.15.512383}, employs a two-level Bayesian matrix factorization model to jointly generate hierarchical clustering and infer gene signatures for each cluster. Notably, among these methods, only scDEF has the capability to handle batch effects. However, it generates a two-level hierarchy rather than a binary tree, posing challenges for comparisons with methods such as scTree.



